Jointly Identifying and Fixing Inconsistent Readings from Information Extraction Systems

KGCleaner is a framework to identify and correct errors in data produced and delivered by an information extraction system. These tasks have been understudied and KGCleaner is the first to address both. We introduce a multi-task model that jointly learns to predict if an extracted relation is credible and repair it if not. We evaluate our approach and other models as instance of our framework on two collections: a Wikidata corpus of nearly 700K facts and 5M fact-relevant sentences and a collection of 30K facts from the 2015 TAC Knowledge Base Population task. For credibility classification, parameter efficient simple shallow neural network can achieve an absolute performance gain of 30 $F_1$ points on Wikidata and comparable performance on TAC. For the repair task, significant performance (at more than twice) gain can be obtained depending on the nature of the dataset and the models.

==> section/commented-approach.tex <==
\begin{comment}
\section{Approach from old paper}
We describe each of our models and training procedure to tackle lack of labeled data by training our models on larger Wikidata dataset and applying trained models to test on smaller TAC dataset. As shown in Figure \ref{fig:crmtarch}, the input to the system is a fact represented as a triple $\langle Wolfgang Amadesu Mozart,per:placeOfBirth,Salzburg\rangle$ where \textit{s} is the subject, \textit{r} the relation, and \textit{o} the object, along with an optional provenance text; this might be a reference to a document or a portion of a document. The system has two outputs: a credible or not credible judgment, and a suggested correct fact if judged not credible. When provenance text is missing, we identify and fetch relevant sentences and encode sentence in features and pass it to the model for joint classification. We consider only those facts for which we could fetch at least one sentence.
%\todo{is it always just a document? Do you ever use the offsets provided in the tac data?} 
%\todo[inline]{Clarify that the subject aliases were used to fetch the page of similar titles or titles with subject aliases only object and predicate aliases were used to fetch provenance sentences because wikipedia document talk about a topic in details and assuming subject and subject alases fetch document of similar kind. Need to recall and rephrase complete intuition.}
%\todoFF[inline]{\colorbox{green}{DONE.} somewhere in this section, citet Ferraro et al. (2014) for the FrameNet annotations, i.e., CAW}
\subsection{Phase 1 - Finding relevant sentences}
\label{sec:fetchrelevantsentence}

	We do not make strong assumptions on the availability of sentence-level provenance information. %as the provenance text to support an extracted fact might be optional and not available. %
	We consider two cases---when provenance is available (in TAC-KBP), and when it is not (in Wikidata). %
	Wikidata~\cite{vrandevcic2014wikidata} facts have document-level, but not sentence level, provenance. %
	We provide highly effective methods for approximately finding this sentence-level provenance. %
	%To find candidate provenance text within a given document, we analyze semantic parses of sentences in the document.
	TAC-KBP facts have sentence-level provenance, which we use directly. %

\textbf{Document selection:} For each of the fact from Wikidata we used the Wikipedia link pointing to the subject of the fact. Such a process naturally handles the challenge of entity disambiguation. 
%use exact string match on Wikipedia to retrieve information about the subject. 
%We additionally created a database of subjects, objects, and predicates with their corresponding aliases and use it to fetch more documents when there is an alias match. 


\textbf{Sentence selection:} Within a provenance document, we consider a sentence to be relevant if it satisfies any of the following criteria: (i) the subject or object or one of their aliases is mentioned in the sentence; (ii) a paraphrase of the object is mentioned in the sentence; (iv) the predicate or an alias is mentioned in the sentence; (iv) or the sentence triggers (i.e., is annotated by) a FrameNet frame~\cite{ferraro2014concretely} for the predicate. %
For objects we also considered aliases when the object was paraphrased; we used the ParaPhrase Database~\cite{ganitkevitch2013ppdb}. 
We consider these criteria to be inspired by both semantic considerations, as represented by the semantic frame and relation alias criteria, and discourse considerations, as represented by the subject and object paraphrase criteria. %

%\begin{itemize}
%\item if the subject is mentioned in the sentence
%\item if an alias of the subject is mentioned in the sentence
%\item if the object is mentioned in the sentence
%\item if an alias of the object is mentioned in the sentence
%\item if an paraphrase of the object is mentioned in the sentence
%\item if the predicate is mentioned in the sentence
%\item if an alias of the predicate is mentioned in the sentence
%\item if the sentence triggers a frame from FrameNet for the predicate under consideration
%\end{itemize}


\textbf{Frame based sentence selection:} We manually mapped Wikidata relations to FrameNet frames and judged a sentence to be relevant when it triggered one of the mapped frames for the predicate. 

%We used the sentences only when the frame was entailed by the sentence. 
%\subsection{Sentences as Average Bag-of-Embeddings \& features}





 \label{sec:approach}
% \begin{figure*}[t]
% \centering
% %\fbox{
% %\subfigure{\includegraphics[scale=0.55]{./image/kgcleaner1.png}}
% %\subfigure{\includegraphics[scale=0.55]{./image/kgcleaner_gumble_shared.png}}
% %subfigure{\includegraphics[scale=0.55]{./image/kgcleaner_gumble_shared_concat_repair.png}}'
% \begin{subfigure}[t]{.32\textwidth}
%   \includegraphics[width=\textwidth]{./image/kgcleaner1_input.png}
%   \caption{Basic model}
%   \label{fig:all_models:basic_kgcleaner}
% \end{subfigure}
% ~
% \begin{subfigure}[t]{.32\textwidth}
%   \includegraphics[width=\textwidth]{./image/kgcleaner_gumble_shared_input.png}
%   \caption{Shared noise model}
%   \label{fig:all_models:sn_kgcleaner}
% \end{subfigure}
% ~
% \begin{subfigure}[t]{.32\textwidth}
%   \includegraphics[width=\textwidth]{./image/kgcleaner_gumble_shared_concat_repair_input.png}
%   \caption{Shared noise + repair concatenation model}
%   \label{fig:all_models:repair_concat_kgcleaner}
% \end{subfigure}
% %}
% \caption{Novel classifier models to determine credibility and repair errors of the extracted fact produced by the information extraction system. This classifier is denoted by ``\textit{f}'' in Figure \ref{fig:crmtarch}.}
% \label{fig:all_models}
% \end{figure*}

%\todoFF{\colorbox{green}{not calculated.}how many/what pct are OOV?} 
%\todo[inline]{Some cool name for each of the model like Reparameterized representation}
% like FrameNet. 


\subsection{Phase 2 - Jointly Learning Credibility and Repair}
\label{sec:models}
\textbf{Sentence Representation:} We used pre-trained word embeddings and binary features to featurize sentences.  For each fact we compute the average of the embeddings of the words in its provenance sentences, using a zero-vector for out-of-vocabulary words. We found averaging the word embeddings with the relation context gave reasonable performance and it allowed us to focus on our core task of repairing and determining credibility. {\color{red}As stated in Table \cref{tab:credibilityperformance} and \cref{tab:something}, we compared with CNN and LSTM for sentence representation and found it to perform poorly and overall they resulted in higher computation cost.}

We additionally converted the selection criteria mentioned in \cref{sec:catelogingIEsystemerrors} into binary features. We combined binary features with bit-wise OR-ing when more than one sentence is retrieved. %These features align with the error types  described in \cref{sec:catelogingIEsystemerrors}, and help identify which provenance sentences do not support the object and/or entail the relationship. 
We concatenate the average word embedding with the computed binary features. \\

\noindent\textbf{Models:} We describe three novel models to jointly learn credibility classification and repair: (i) a basic \SYSNAME{}, (ii) \SYSNAME{} with Gumbel, (iii) \SYSNAME{} with Gumbel and context.

%\subsubsection{\SYSNAME{} Basic}

\paragraph{Model 1 - \SYSNAME{} Basic.}
A feedforward MLP was employed to learn distribution of the credibility and repair tasks with shared parameters. %\todo{this was all said before} As shown in Figure \ref{fig:crmtarch} the input to the system is a fact with a document id as provenance. We fetch relevant sentences using the previously mentioned approach. We combine all the fetched sentences to form a text blob. We use pre-trained word embedding to convert the text blob to a dense representation and take average over text blob. Additionally, we extract binary features from the sentences for the network model to distinguish credible fact from incredible facts. 
%and also learn if a relation could be recommended to be repaired. 
As shown in Equation \ref{eq:hiddenlayer}, each layer learns an abstract representation from the previous one.
 \begin{gather}
 \boldsymbol{h}^{(0)}  = \quad \boldsymbol{x}_{f} \\
 \label{eq:hiddenlayer}
 \boldsymbol{h}^{(i)} = \quad g^{(i)}(\boldsymbol{W}^{(i)}\boldsymbol{h}^{(i-1)}+\boldsymbol{b}^{(i)})\\ % \quad i \in \{1,2\}\\
 \hat{y}_{c}  = \quad \sigmoid(\boldsymbol{W}_{cred}^{(last)}\boldsymbol{h}^{(last)}+\boldsymbol{b}^{(last)}) \\
 \hat{\boldsymbol{y}}_{r}  = \quad \softmax(\boldsymbol{W}_{repair}^{(last)}\boldsymbol{h}^{(last)}+\boldsymbol{b}^{(lst)})
 %&\boldsymbol{g}^{(i)} & = & \quad \max\{0,\boldsymbol{h}^{(i)}\}\\
 \end{gather}


%{
%\vspace{-2em}
%\begin{subequations}
%\begin{tabularx}{\textwidth}{p{2.5in}p{3in}}
%\begin{equation}
%\mathbf{h}^{(0)}  =  \mathbf{x}_{f}
%\vspace{-.5in}
%\end{equation}
%&
%\begin{equation}
%\mathbf{h}^{(i)} = g^{(i)}(\mathbf{W}^{(i)}\mathbf{h}^{(i-1)}+\mathbf{b}^{(i)})
%\vspace{-.5in}
%\label{eq:hiddenlayer}
%\end{equation} \\ % \quad i \in \{1,2\}\\
%\begin{equation}
%\hat{y}_{c}  = \sigma(\mathbf{W}_{\textit{cred}}^{(\textit{last})}\mathbf{h}^{(\textit{last})}+\mathbf{b}^{(\textit{last})})
%\end{equation}
%& %\\
%\begin{equation}
%\hat{{y}}_{r}  = \softmax(\mathbf{W}_{\textit{repair}}^{(\textit{last})}\mathbf{h}^{(\textit{last})}+\mathbf{b}^{(\textit{last})})
%\end{equation}
%%&\boldsymbol{g}^{(i)} & = & \quad \max\{0,\boldsymbol{h}^{(i)}\}\\
%\end{tabularx}
%\vspace{-2em}
%\end{subequations}
%
%}%

\noindent
Here $i$ is the number of layers; variables with the $\textit{last}$ superscript indicate parameters and values from the last hidden layer. 
%We set $g$ to introduce non-linearity. We set $g$ to $\tanh$. 
We set each $g^{(i)}$ to $\tanh$ to introduce non-linearity.
Each $\textbf{x}_f$ is the input to the system and has dimension $e$+$n$ where $e$ is the word-embedding dimension and $n$ is the number of features. The dimension of $\textbf{W}^{(i)}$ except for the last layer is $(e+n)\times(e+n)$. The dimension of $\textbf{W}^{(i)}_{cred}$ and $\textbf{W}^{(i)}_{repair}$ is $1 \times (e+n)$ for binary classification and $r \times (e+n)$ to obtain a probability distribution over all relations. $b^{(i)}$, and $b^{(last)}$ are the biases vectors. We use a sigmoid ($\sigma$) function for binary credibility classifier and softmax for relation classification.
For credibility, we minimized regularized binary cross entropy; for relation repair, we minimized a categorical cross entropy. Note that if $h^{(0)} = h^{(\textit{last})}$, then we are using logistic regression classifiers. 

%While our framework has the flexibility to use a range of sentence representation and classification models, from sophisticated neural networks (e.g., CNN, RNN) to simple linear regression, 
We opted for MLPs as a basic model (\cref{fig:all_models:basic_kgcleaner}) due to their simplicity, e.g., fewer parameters. We note that MLPs have been successful in verifying news in the 2017 Fake News Challenge \cite{fnc}, where two of the top three teams used them.

%\todo[inline]{What about other activation functions?}

%\subsubsection{\SYSNAME{} with re-parameterization}
\label{sec:kgc-gumbel}
%\todo[inline]{Explain Gumbel-Softmax}
%\todo[inline]{Write why Gumbel-Softmax works with citations}
\paragraph{Model 2 \& 3 - \SYSNAME{} with re-parameterization.}

{\color{red} We also experimented with computing the outer product of a relation one-hot vector and the concatenated features; this allowed the network to be aware of the original extracted relation.}

We extend the KG-Cleaner Basic model with a layer of discrete
stochastic nodes as a hidden layer using a \textit{re-parameterization
trick}, where samples $\{z_k\}$ from a fixed distribution are transformed to reparametrize hidden discrete latent variables and still allow backpropagation; this process also helps lower the variance of the estimator \cite{maddison2016concrete,jang2016categorical}. Re-parameterization has been used before when the intermediate stochastic node are continuous random variables but its difficult for discrete random variables as they introduce non-differentiable operations. A solution is to reparametrize and approximate the discrete component $y_k \propto \exp{\left(\tau^{-1}(z_k + \log \pi_k)\right)}$. Each $z_k$ is a sample from a Gumbel(0,1) distribution, $\pi_k$ are the probability parameters, and $\tau$ is a free parameter that governs the entropy of the approximation. Following Jang et al. \shortcite{jang2016categorical}, we call this a Gumbel-Softmax. %
This re-parameterization has recently started to get  for natural language tasks \cite{poerner2018interpretable,chen2018smaller,choi2018learning,guo2018inducing,lu2017best}. However, to the best of our knowledge, our framework is the first to propose the use of Gumbel-Softmax as a stochastic layer to maintain knowledge graphs by identifying and correcting errors.

In our framework the discrete output is produced by the relation classification. %
The classification output is the argmax of the probability distribution represented as a one-hot vector, and is hence discrete. 
Such a function directly cannot be used as a hidden layer inside the neural network as the back propagation due to the non-differentiability the argmax introduces. We use a Gumbel-Softmax layer to support back propagation as shown in Eq. \ref{eq:gumbel_softmax}, with $\mathcal{\boldsymbol{n}}_i$ as a vector of Gumbel samples:
%One solution to this problem is to use a Gumbel-Softmax~\citep{jang2016categorical} reparametrization, which approximates the discrete distribution such that back propagation is possible. 
% Preview source code for paragraph 0
\begin{eqnarray}
	\mathcal{\mathcal{G}}\left(\boldsymbol{h}^{\left(i\right)}\right) & = & \softmax{\left(\left(\log\left(\boldsymbol{h}^{\left(i\right)}\right)+\boldsymbol{z}\right)\cdot\tau^{-1}\right)}
	\label{eq:gumbel_softmax}
\end{eqnarray}

%Here $ \approx -\log(\log(\mathcal{U}(0,1))$ is the Gumbel sample. $\tau$ is the temperature which controls the approximation between discrete and continuous approximation. %Smaller the value of $\tau$ closer the approximation to one-hot vector (i.e discrete distribution).

As shown in \cref{fig:all_models:sn_kgcleaner,fig:all_models:repair_concat_kgcleaner}, $\mathcal{G}$ represents the Gumbel-Softmax layer (Eq. \ref{eq:gumbel_softmax}) where the input logits are mixed with a sample of the same dimension as logits from a Gumbel distribution ($\mathcal{\boldsymbol{z}}_i$). As actual representation $\boldsymbol{h}^{(i)}$ gets mixed with $\boldsymbol{z}^{(i)}$, we call the new representation $\mathcal{G}(\boldsymbol{h}^{(i)})$ as a \textit{noisy representation}. Empirically (\cref{sec:experiments}) such a noisy representation helps to generalize the model better by training on an encyclopedic domain (Wikipedia) and applying it to a news domain (TAC). %
\Cref{fig:all_models:sn_kgcleaner} depicts the model where the noisy representation is shared between the task without reference to the features obtained from the previous layer. Meanwhile, \cref{fig:all_models:repair_concat_kgcleaner} concatenates the shared noisy representation and the abstraction from the previous layer prior to a final relation repair. %Such a design better support the learning of the repair task. 

\textbf{Joint objective function}: For relation classification we used cross-entropy as loss function and for credibility we used binary loss function as follows:
\begin{eqnarray}
	\mathcal{L}_{joint} & = & -\stackrel[i=1]{k}{\sum}y_{r}^{(i)}log\hat{y}_{r}^{(i)}\\
	&  & +\left(-y_{c}^{(0)}logy_{c}^{(0)}+(1-y_{c}^{(0)})log\left(1-y_{c}^{(0)}\right)\right)
\nonumber
\end{eqnarray}

Here superscript on $y_c$ or $y_r$ indicates corresponding class.
\subsection{Training and Negative Sampling}
\label{sec:negativesampling}

We trained all \SYSNAME{} variants using stochastic gradient descent with a momentum of 0.9 ~\cite{sutskever2013importance} and a decay rate of 10$^{-6}$. We initialized the models with Xavier Uniform initialization~\cite{glorot2010understanding} and used back propagation to learn the parameters. 

%Both tasks utilize a from common representation. 
%we used Wikipedia document pointed to by Wikidata fact and use negative sampling.
%, similarly randomly replacing the set of provenance sentences and the object.

Since we have only test data for small dataset like TAC, we train our models on large dataset like Wikidata and apply trained model on test dataset for TAC. Since our Wikidata facts provide only positive examples, we generated ``faux facts'' for training from them by first fixing the subject and then replacing the relation and object with a randomly selected ones and associating a randomly selected provenance text segment from one of the positive examples. %
In negative sampling we do not prefer any particular relation or object over other, but follow a uniform distribution to randomly pick relation, object, and provenance. We label all positive examples as credible, with the ``repaired' relation the same as the input relation (i.e., encourage the system to learn the right relations when a fact is credible). Negative instances are not credible and a special ``cannot repair'' relation.  During training, we used a balanced batch with an equal number of positive and negative examples. Despite any seeming simplicity in the negative sampling, as we discuss in \cref{sec:experiments}, this approach led to large improvements in multiple domains. We also tried different combinations of replacing the object, relation and provenance (e.g., only relation, only object and provenance, etc.) but found above described sampling to perform better. %

We trained each of the models on our Wikidata training set and used pre-trained 100 dimensional Glove word embeddings.
%uniform distribution to randomly pick relation, object or provenance to perform better.}
%
%\todoFF{\colorbox{green}{DONE}. \colorbox{green}{No experiments}Was this at all experimented with?}
%We consider equal number of positive and negative facts in each batch.
%\todo[inline]{No experiments conducted to study portion of positive and negative in batch size. We assumed the batch is balanced.}

\end{comment}


==> section/commented-intro-ending.tex <==
%We additionally identified the influential features beside embedded representation and validated our observations against multiple dataset of diverse characteristic, and with a comparison against state-of-the-art methods  .

        %We demonstrate supervised training on large knowledge graph (like WikiData) with positive examples and negative sampling along with expert evaluated LDC corpus. We show the effectiveness of using structured semantic representations for provenance retrieval (when provenance is missing) and effect of different kinds of relation mapping (\cref{sec:ablationstudy}).  
%\end{itemize}

%{\color{red}We found that significant improvement can be achieved by adding noise during training, and that \SYSNAME{} models can perform quite well when trained using Negative Sampling and tested on extracted facts using embeddings and semantic parses.}
%\begin{figure*}
%	\centering
%	
%	\begin{minipage}{.6\textwidth}
%		\flushleft
%		\includegraphics[scale=0.33]{./image/arch4.png}
%		%\includegraphics[width=1.0\linewidth]{./image/arch4.png}
%		\caption{Overview of \SYSNAME's joint credibility and repair model.} %
%		%\NoteFF{I thought each sentence was predicted as credible or not...}}
%		\label{fig:crmtarch}
%	\end{minipage}%}
%\hfill
%	\begin{minipage}{.4\textwidth}
%		\centering
%		\includegraphics[scale=0.8]{./image/tac_human_error_chart.png}
%		\captionof{figure}{Frequency count vs. TAC error types. The error analysis was performed on facts extracted by a real IE system.%
%			\label{fig:previous-tac-errors}
%		}
%	\end{minipage}
%\end{figure*}

%\todo[inline]{AP: In diagram Concat repair is missing one layer before concatination. Will fix later.}
% \begin{figure*}[t]
%	\centering
%	\begin{subfigure}[t]{\textwidth}
%		\centering
%		\includegraphics[scale=0.45]{../image/arch4.png}
%		%\includegraphics[width=1.0\linewidth]{./image/arch4.png}
%		\caption{Overview of \SYSNAME's joint credibility and repair model.} %
%		%\NoteFF{I thought each sentence was predicted as credible or not...}}
%		\label{fig:crmtarch}
%	\end{subfigure}
%\par\bigskip % force a bit of vertical whitespace
%	%\fbox{
%	%\subfigure{\includegraphics[scale=0.55]{./image/kgcleaner1.png}}
%	%\subfigure{\includegraphics[scale=0.55]{./image/kgcleaner_gumble_shared.png}}
%	%subfigure{\includegraphics[scale=0.55]{./image/kgcleaner_gumble_shared_concat_repair.png}}'
%	\begin{subfigure}[t]{.25\textwidth}
%		%\includegraphics[width=0.5\textwidth]{./image/kgcleaner1_input.png}
%		\includegraphics[scale=0.38]{../image/kgcleaner1_rightangle.png}
%		\caption{Basic model}
%		\label{fig:all_models:basic_kgcleaner}
%	\end{subfigure}
%	~
%	\begin{subfigure}[t]{.33\textwidth}
%		%\includegraphics[width=0.5\textwidth]{./image/kgcleaner_gumble_shared_input.png}
%		\includegraphics[scale=0.38]{../image/kgcleaner2_rightangle.png}
%		\caption{\SYSNAME{} + Gumbel}
%		\label{fig:all_models:sn_kgcleaner}
%	\end{subfigure}
%	~
%	\begin{subfigure}[t]{.33\textwidth}
%		%\includegraphics[width=0.5\textwidth]{./image/kgcleaner_gumble_shared_concat_repair_input.png}
%		\includegraphics[scale=0.38]{../image/kgcleaner3_rightangle.png}
%		\caption{\SYSNAME{} + Gumbel + Residual Connection}
%		\label{fig:all_models:repair_concat_kgcleaner}
%	\end{subfigure}
%	%}
%	
%	\caption{Novel classifier models to determine credibility and repair errors of the extracted fact produced by the information extraction system. This classifier is denoted by ``\textit{f}'' in Figure \ref{fig:crmtarch}.}
%	\label{fig:all_models}
%\end{figure*}



%\begin{minipage}{\columnwidth}
%\begin{figure}[t]
%	\centering
%	\includegraphics[scale=0.3]{./image/arch4.png}
%	%\includegraphics[width=1.0\linewidth]{./image/arch4.png}
%	\caption{Overview of \SYSNAME's joint credibility and repair model.} %
%	%\NoteFF{I thought each sentence was predicted as credible or not...}}
%	\label{fig:crmtarch}
%\end{figure}
%\begin{figure}
%	\centering
%	\includegraphics[scale=0.7]{./image/tac_human_error_chart.png}
%	\captionof{figure}{Frequency count vs. TAC error types. The error analysis was performed on facts extracted by a real IE system.%
%		\label{fig:previous-tac-errors}
%	}
%\end{figure}
%\end{minipage}



%\todo[inline]{Find a way to introduce frames like ``Frames from FrameNet contains value information. Each of the frame can be considered as role where the the frame elements becomes the argument of the role. ''}

%There has been many research to extract information from the text documents and have been show to work on web scale \citet{}. However, the IE systems are not perfect and hence makes mistakes. The errors are sipped in the constructed knowledge base. This reduces the utility of the knowledge base. The best of our knowledge very limited work has been done to clean the knowledge base and no work have studied to improve the quality of knowledge base by repairing erroneous facts. In this paper, we fill this gap. 

%We introduce a credibility and repair multi-task model (CRMT). %
%Outlined in Figure \ref{fig:crmtarch}, this model jointly learns how to detect credible vs. non-credible facts and how to propose potential repairs to \todoFF{Is this (qualifying to ``non-credible facts'' true?}non-credible facts. Unlike previous approaches\todoFF{citet a couple, as necessary}, our single CRMT model is standalone and does not use an ensemble of IE systems nor does it rely on Web search engines. \todoFF{this sentence wasn't finished, but I'm not sure where it was going; it seems to repeat what else has already been said}We jointly train our model on two related task of credibility and repair of the facts where a incorrect fact need a repair when possible and correct fact \todo{????} 





==> section/discussion.tex <==
no longer used

==> section/supplementary_material <==
\subsection{Hyper tuning}
We tried the following values: for learning rate, \{10$^{-1}$,10$^{-2}$,10$^{-3}$,10$^{-4}$,10$^{-5}$\}; for Lasso regularization, \{10$^{-2}$,10$^{-3}$,10$^{-4}$,10$^{-5}$,10$^{-6}$\}; for the number of epochs, \{5, 25, 50, 100\}. %
We used a fixed dropout of 0.2. %

\subsection{Logistic Regression as classifier.}
We followed the same procedure to train Logistic Regression (LR) models as we did for our models, replacing our re-parameterized model (Gumbel-Softmax) with LR.  We then evaluated its performance with different sentence representations on the credibility and relation tasks. \Cref{tab:credibilityperformanceLR} shows the performance of LR is significantly worse than \SYSNAME{}'s shared re-parameterize model. LR's poor performance stems from its lack of expressibility in capturing the task's subtle nuances. For credibility, LR's performance is similar, however the binary vector performs relatively better, indicating the importance of lexical words in the classification task. LR performance drops by nearly $\sim 70\%$ (comparing F1 columns for Wikidata-test and TAC) when tested on the TAC domain. A similar trend is seen in performance on the repair task. The micro score is relatively high compared to macro, as the logistic regression models frequently predicted ``no repair possible''. TAC results are similar.

%\input{../table/credibility_performanceLR.tex}
%\input{../table/credibility_performance_naive_bayes.tex}
%\input{../table/repair_performanceLR.tex}
%\input{../table/repair_performance_naive_bayes.tex}

\input{../table/wikidata_relation.tex}


\input{../table/credibility_performance_short.tex}
\input{../table/repair_performance_short.tex}


%\subsubsection{Cleaning using Graph structure}

\paragraph{Cleaning using Graph structure.}
Motivated by standalone systems, it makes sense to compare our language based approach with existing methods like DistMult and ComplEx, which learn embeddings for entities and relations. 
Our goal is to understand the embedding produced by these methods which distinguish correct from incorrect facts. Both have been well studied for the link-prediction task. 
Link prediction and fact credibility prediction are different: the former involves ranking possible entity objects, given a subject and relation, while the latter classifies the fact as correct or incorrect. %
%\textbf{Dataset, hyperparameters, and evaluation:} 
As both systems train on positive examples, like our models we train them on Wikidata positive examples. 
We hyper-tuned the models as described above and chose the setting that performed  best on the Wikidata validation set. 
We tested the models on Wikidata-test. We computed the score of the fact using embeddings of subject, relation and object and thresholded the value to 0.5; if the score is greater than 0.5 we considered fact to be credible. 

%\textbf{Discussion:}
Table \ref{tab:credibilityperformance} shows the performance of DistMult and ComplEx on credibility classification for Wikidata test. 
The trained models cannot be applied to TAC, as indicated by NA, because both models make a closed-world assumption: the models are not aware of the entities present in different knowledge bases, like TAC, and there is no TAC-specific training data. 
Moreover, we use TAC as an additional dataset to evaluate the method we are not training, either ours or other models, on the TAC dataset. 
Compared to our model, both  perform poorly with ComplEx being slightly better than DistMult. We believe this improvement is due to the way that the ComplEx tries to embed the entities and relations. %
%\textcolor{purple}{Based on the performance scores, the reason DistMult and ComplEx perform poorly is that the embeddings they learn are well suited for a link prediction task and not a fact credibility one.} %

%\sout{\textbf{Discussion:} Table \ref{tab:credibilityperformance} shows the performance of DistMult and ComplEx on credibility classification for Wikidata-test. The trained models cannot be applied to TAC, as indicated by NA, because both models make a close-world assumption, and hence the models are not aware of the entities present in different knowledgebases, like TAC. Moreover, we use TAC as an additional dataset to evaluate the method we are not training, either ours or other models, on the TAC dataset. Compared to our model, both  perform poorly with ComplEx being slightly better than DistMult. We believe this improvement is due to the way the ComplEx tries to embed the entities and relations.} %Also, based on the performance scores, the reason DistMult and ComplEx perform poorly is thaT the embeddings they learn are well suited for a link prediction task and not a fact credibility one. 

%\subsubsection{Logistic Regression as classifier}


%{\color{red} binary vectors perform better than other LR based models}


A similar trend is seen when comparing \SYSNAME{} with DistMult and ComplEx. Their performance is poor, and help demonstrate important empirical differences in learning representations for link prediction vs. fact credibility. These differences also highlight the utility of language as an additional source of information to verify the credibility of the fact. 


==> table/ablation_tables.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[]
	\centering \resizebox{.99\textwidth}{!}{ \begin{tabular}{|c|c|c|c||c|c|c||c|c|c||c|c|c|} \hline %\multirow{2}[4]{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Credibility}} & \multicolumn{3}{c|}{\textbf{Credibility}} & \multicolumn{3}{c|}{\textbf{Credibility}} \\ %\multicolumn{1}{|c|}{} & \multicolumn{3}{c|}{\textbf{TACRED2}} & \multicolumn{3}{c|}{\textbf{TAC-2017}} & \multicolumn{3}{c|}{\textbf{TAC-2015}} \\ \textbf{Rep.} & \textbf{Comb.} & \textbf{Clf.} & \textbf{Lex.} & \multicolumn{3}{c||}{\textbf{TACRED}} & \multicolumn{3}{c||}{\textbf{TAC-17}} & \multicolumn{3}{c|}{\textbf{TAC-15}} \\ \hline %\multicolumn{1}{|c|}{} & \multicolumn{1}{p{4.055em}|}{\textbf{p }} & \multicolumn{1}{p{4.055em}|}{\textbf{r }} & \multicolumn{1}{p{4.055em}|}{\textbf{f1 }} & \multicolumn{1}{p{4.055em}|}{\textbf{p }} & \multicolumn{1}{p{4.055em}|}{\textbf{r }} & \multicolumn{1}{p{4.055em}|}{\textbf{f1 }} & \multicolumn{1}{p{4.055em}|}{\textbf{p }} & \multicolumn{1}{p{4.055em}|}{\textbf{r }} & \multicolumn{1}{p{4.055em}|}{\textbf{f1 }} \\ & & & & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\ \hline %\textbf{LSTM-TEXT} & 63.90 & 100.00 & 77.97 & 46.59 & 90.31 & 52.97 & 39.05 & 57.11 & 46.38 \\ %\hline %\textbf{Declare} & 63.90 & 100.00 & 77.97 & 36.03 & \textbf{100.00} & 52.97 & 26.87 & \textbf{100.00} & 42.36 \\ %\hline %\textbf{\SYSNAME} & \textbf{78.68} & \textbf{99.30} & \textbf{87.80} & 48.59 & 84.21 & \textbf{61.62} & \textbf{46.15} & \textbf{76.06} & \textbf{57.44} \\ BoW embedding & No & MLP & No & 63.9 & 100.0 & 77.97 & 36.02 & \textbf{99.95}& 52.96 & 26.87 & \textbf{100.0}& 42.36 \\
		
		%\textbf{\SYSNAME}+C & 68.04 & 42.93 & 52.64 & 36.03 & 100 & 52.97  & 0 & 0 & 0 \\
		 \textbf{Rep.} & \textbf{Comb.} & \textbf{Clf.} & \textbf{Lex.} & \multicolumn{3}{c||}{\textbf{TACRED}} & \multicolumn{3}{c||}{\textbf{TAC-2017}} & \multicolumn{3}{c|}{\textbf{TAC-2015}} \\
			\hline
			& & &   & \textbf{Macro} & \textbf{Micro} & \textbf{MRR} & \textbf{Macro} & \textbf{Micro} & \textbf{MRR} & \textbf{Macro} & \textbf{Micro} & \textbf{MRR} \\
			\hline
		BoW embedding & Yes & MLP & No  & 64.05 & 13.11 & 21.76 & 37.46 & 36.63 & 37.04  & 26.69 & 50.48 & 34.92 \\
		BoW embedding & No & MLP & Yes  & 63.87 & 99.80 & 77.89 &37.38  & 51.16  & 43.19  & 25.89 & 56.73  & 35.56 \\
		%\textbf{\SYSNAME}+T & 63.87 & 99.80 & 77.89 & 37.38 & 51.16 & 43.19  & 25.89 & 56.73 & 35.56 \\
		BoW embedding & Yes & MLP & Yes  &\textbf{78.68} & \textbf{99.30} & \textbf{87.80} & \textbf{48.59} & 84.21 & \textbf{61.62} & \textbf{46.15} & 76.06 & \textbf{57.44} \\
		Bi-LSTM & Yes & MLP & Yes  &  63.92 & 96.57 & 76.92 & 35.91 & 58.77 & 44.58 & 26.28 & 69.27 & 38.11\\
		\hline
	\end{tabular}%
}
	\caption{Consistency performance ablation study, where "Rep." is representation, "Comb." is belief and provenance combination, "Clf." is classifier, and "Lex." is lexical features as TF-IDF vector.}
	\label{tab:consistencyPerformanceAblation}%
\end{table*}%

\todo{Table 6 please check the macro and micro numbers. What are the classes being averaged over (in email please enumerate them)}

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[]
	\centering
	\resizebox{.99\textwidth}{!}{
		\begin{tabular}{|c|c|c|c||c|c|c||c|c|c||c|c|c|}
			\hline
		 \textbf{Rep.} & \textbf{Comb.} & \textbf{Clf.} & \textbf{Lex.} & \multicolumn{3}{c||}{\textbf{TACRED}} & \multicolumn{3}{c||}{\textbf{TAC-2017}} & \multicolumn{3}{c|}{\textbf{TAC-2015}} \\
			\hline
			& & &   & \textbf{Macro} & \textbf{Micro} & \textbf{MRR} & \textbf{Macro} & \textbf{Micro} & \textbf{MRR} & \textbf{Macro} & \textbf{Micro} & \textbf{MRR} \\
			\hline
			BoW embedding & No & MLP & No & 0.02 & 0.52 & 0.05 &0.02 &0.16 & 0.06 & 0.03 & 0.52 & 0.05 \\
			%\textbf{\SYSNAME}+C & 0.01 & 0.24 & 0.05 & 0.01 & 0.17 & 0.06  & 0.07 & 0.45 & 0.11\\
			BoW embedding & Yes & MLP & No  & 0.55 & 0.81 & 0.06 & 1.41 & 6.26 & 0.20 &0.28 & 0.48 & 0.06 \\
			BoW embedding & No & MLP & Yes  & 0.37 & 0.78  & 0.08  & 1.10  & 3.65  & 0.10 & 0.9 & 6.05 & 0.19  \\
			
			BoW embedding & Yes & MLP & Yes  & \textbf{2.10}  & \textbf{78.56} & \textbf{0.81}  & \textbf{79.13} & \textbf{84.15} & \textbf{0.91} & \textbf{64.90} & \textbf{75.90} & \textbf{0.85} \\
			Bi-LSTM & Yes & MLP & Yes  & 1.38& 21.33& 0.37 & 0.77 & 3.59 & 0.12 & 0.71 & 3.22 & 0.14 \\
			\hline
		\end{tabular}%
	}
	\caption{Repair performance ablation study with abbreviations as in Table \ref{tab:consistencyPerformanceAblation}.}
	\label{tab:repairPerformanceAblation}%
\end{table*}%





==> table/consistency_performance_new.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
	\centering
	\resizebox{0.99\textwidth}{!}{
	\begin{tabular}{|c|c|c|c||c|c|c||c|c|c||c|c|c|}
		\hline
		%\multirow{2}[4]{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Credibility}} & \multicolumn{3}{c|}{\textbf{Credibility}} & \multicolumn{3}{c|}{\textbf{Credibility}} \\
		%\multicolumn{1}{|c|}{} & \multicolumn{3}{c|}{\textbf{TACRED2}} & \multicolumn{3}{c|}{\textbf{TAC-2017}} & \multicolumn{3}{c|}{\textbf{TAC-2015}} \\
		\textbf{Rep.} & \textbf{Comb.} & \textbf{Clf.} & \textbf{Skip}& \multicolumn{3}{c||}{\textbf{TACRED}} & \multicolumn{3}{c||}{\textbf{TAC-17}} & \multicolumn{3}{c|}{\textbf{TAC-15}} \\
		\hline
		%\multicolumn{1}{|c|}{} & \multicolumn{1}{p{4.055em}|}{\textbf{p }} & \multicolumn{1}{p{4.055em}|}{\textbf{r }} & \multicolumn{1}{p{4.055em}|}{\textbf{f1 }} & \multicolumn{1}{p{4.055em}|}{\textbf{p }} & \multicolumn{1}{p{4.055em}|}{\textbf{r }} & \multicolumn{1}{p{4.055em}|}{\textbf{f1 }} & \multicolumn{1}{p{4.055em}|}{\textbf{p }} & \multicolumn{1}{p{4.055em}|}{\textbf{r }} & \multicolumn{1}{p{4.055em}|}{\textbf{f1 }} \\
		& & & & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
		\hline
		%\textbf{LR + Count} & 63.97 & 83.57 & 72.47 & \textbf{63.87} & 31.25 & 0.24  & 26.83 & 0.60  & 1.17 \\
		%\hline
		%\textbf{LR + Binary} & 63.96 & 83.46 & 72.42 & 63.87 & 31.25 & 0.24  & 26.83 & 0.60  & 1.17 \\
		%\hline
		\textbf{TF-IDF} & No & LR & No & 63.95 & 83.24 & 72.33 & \textbf{57.58} & 30.66 & 14.05 & 22.68 & 15.08 & 18.12 \\
		\hline
		%\hline
		%\textbf{LR+Emb.+SUM} & 63.90 & 99.99 & 77.97 & 63.97 & 0.00  & 0.00  & 0.00  & 0.00  & 0.00 \\
		%\hline
		%\textbf{LR+Emb.+AVG} & 63.90 & 100.00 & 77.97 & 63.97 & 0.00  & 0.00  & 0.00  & 0.00  & 0.00 \\
		
		%\hline\hline
		%\textbf{NB + Count} & 67.84 & 74.06 & 70.81 & 49.64 & 53.10 & 51.31 & \textbf{53.03} & 1.90  & 3.67 \\
		%\hline
		\textbf{Binary} & No & NB & No & 67.84 & 74.06 & 70.81 & 49.64 & 53.10 & 51.31 & \textbf{53.03} & 1.90  & 3.67 \\
		%\hline
		%\textbf{NB + Emb.+AVG} & 64.11 & 99.69 & 78.03 & 100.00 & 0.10  & 0.19  & 0.00  & 0.00  & 0.00 \\
		%\hline
		%\textbf{NB+Emb.+SUM} & 67.18 & 28.19 & 39.72 & 38.65 & 76.60 & 51.37 & 0.00  & 0.00  & 0.00 \\
		%\hline
		%\textbf{NB+TF-IDF} & 70.55 & 52.85 & 60.43 & 0.00  & 0.00  & 0.00  & 29.18 & 59.61 & 39.18 \\
		\hline\hline
		$\spadesuit$  \textbf{LSTM} & No & MLP & No & 63.90 & \textbf{100.00} & 77.97 & 46.59 & 90.31 & 52.97 & 39.05 & 57.11 & 46.38 \\
		\hline
		$\spadesuit$ \textbf{Bi-LSTM} & Yes (W) & MLP & No & 63.90 & \textbf{100.00} & 77.97 & 36.03 & \textbf{100.00} & 52.97 & 26.87 & \textbf{100.00} & 42.36 \\
		\hline
		\textbf{BERT} & Yes (S) & MLP & Yes & 67.79  & 65.12  & 66.47  & 48.09 & 90.02  & 62.69  &  51.49   & 55.97  & 53.88  \\
		\hline
		\textbf{BoW embedding} & Yes (S) & MLP & Yes & \textbf{78.68} & 99.30 & \textbf{87.80} & 48.59 & 84.21 & \textbf{61.62} &  46.15  & 76.06 & \textbf{57.44} \\
		%\textbf{\SYSNAME}(LSTM) &  63.92 & 96.57 & 76.92 & & &  & 26.28 & 69.27 & 38.11\\
		%\hline\hline
		%\textbf{\SYSNAME}+nothing & 63.9 & 100.0 & 77.97 & 36.02 & 99.95& 52.96 & 26.87 & 100.0& 42.36  \\

		%\textbf{\SYSNAME}+C & 68.04 & 42.93 & 52.64 & 36.03 & 100 & 52.97  & 0 & 0 & 0 \\
		%\textbf{\SYSNAME}+A & 64.05 & 13.11 & 21.76 & 37.46 & 36.63 & 37.04  & 26.69 & 50.48 & 34.92 \\
		%\textbf{\SYSNAME}+T & 63.87 & 99.80 & 77.89 &37.38  & 51.16  & 43.19  & 25.89 & 56.73  & 35.56 \\
		%\textbf{\SYSNAME}+A+T &\textbf{78.68} & \textbf{99.30} & \textbf{87.80} & 48.59 & 84.21 & \textbf{61.62} & \textbf{46.15} & \textbf{76.06} & \textbf{57.44} \\
		\hline
		
	\end{tabular}%
}
	\caption{Consistency performance from our framework's models ("Rep." for representation, "Comb." for belief and provenance combination, "Clf." for classifier, "Skip" for skip connection; see \cref{sec:experiments:components} for a detailed explanation of the values). We indicate the state-of-the-art credibility model with $\spadesuit$.}
	\label{tab:consistencyPerformance}%
\end{table*}%


==> table/credibility_performance.tex <==
% all models included
% Table generated by Excel2LaTeX from sheet 'Credibility'
\begin{table*}[t] \small
  \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
    \hline
          & \multicolumn{3}{c|}{\textbf{Wikidata Test (WD)}} & \multicolumn{3}{c|}{\textbf{TAC}} \\
    \hline
          & \multicolumn{1}{c|}{\textbf{precision}} & \multicolumn{1}{c|}{\textbf{recall}} & \multicolumn{1}{c|}{\textbf{f1}} & \multicolumn{1}{c|}{\textbf{precision}} & \multicolumn{1}{c|}{\textbf{recall}} & \multicolumn{1}{c|}{\textbf{f1}} \\
    \hline
    %LR + count vector & 0.501 & 0.536 & 0.518 & 0.312 & 0.478 & 0.378 \\
    LR + Binary Vector & 0.502 & 0.628 & 0.558 & 0.294 & 0.590 & 0.392 \\
    %LR + sum word embedding & 0.500 & 0.516 & 0.508 & 0.290 & 0.452 & 0.353 \\
    LR + Average word embedding & 0.502 & 0.506 & 0.504 & 0.286 & 0.526 & 0.371 \\
    %LR + TFIDF & 0.501 & 0.536 & 0.518 & 0.312 & 0.480 & 0.378 \\
    \hline\hline
    DistMult & 0.577 &	0.544 &	0.560 &	NA &	NA &	NA \\
    ComplEx &0.583&	0.617&	0.580	&NA	&NA	&NA\\
    \hline\hline
    MLP-1 & 0.49 & 0.99 & 0.67 &  & & \\
    MLP-2 & 0.49 & 1.00 & 0.67 & & & \\
    CNN-text & & & & &  & \\
    LSTM-text & 0.50& 0.96& 0.66& 0.30&0.99 &0.47 \\
    LSTM-text & 0.50& 0.99& 0.66& 0.30&0.99 &0.47 \\
    Declare(2018)   & 0.80& 0.99& 0.89& 0.31&0.33 &0.32 \\
    Declare(2018)   &     &     &     &     &     & \\
    \hline\hline

    old \SYSNAME{}, independent training & \textbf{0.995} & 0.820 & \textbf{0.891} & 0.299 & 0.461 & 0.355 \\
    old \SYSNAME{} Basic & 0.975 & 0.819 & 0.890 & 0.289 & 0.462 & 0.355 \\
    \hline\hline
    %\SYSNAME{} (Shared Gumbel Noise) &0.814 &	\textbf{0.935}	&0.870	&\textbf{0.587}	&\textbf{0.876}	&\textbf{0.703} \\
    old \SYSNAME{} (Basic+G) &0.814 &	\textbf{0.935}& 	0.870 &	\textbf{0.587} &	\textbf{0.876} &	\textbf{0.703}  \\
    old \SYSNAME{} (Basic+GC) &0.826&	0.920&	0.870&	0.579&	0.812	&0.676  \\
    \hline\hline

    new \SYSNAME{} (pytroch Basic+GC avg) & 0.9288& 0.9917&0.9592	 &0.2943 & 0.7175 &0.4174   \\
   
    
    %KG Cleaner with 3 layers & \textbf{0.987} & 0.813 & \textbf{0.891} & 0.289 & 0.461 & 0.355 \\
    %KG Cleaner with 4 layers & 0.982 & 0.816 & 0.891 & 0.289 & 0.461 & 0.355 \\
    \hline
    \end{tabular}%
    \caption{Credibility Performance. NA (\textit{Not
        Applicable}) for DistMult and ComplEx as they train on
      fixed set of entities to generate embedding and are trained on WikiData-train, which does not overlap with TAC entities; no embeddings for TAC entities exist. }
  \label{tab:credibilityperformance}%
\end{table*}%





==> table/credibility_performanceLR.tex <==
% LR included
% Table generated by Excel2LaTeX from sheet 'Credibility'
\begin{table*}[h] \small
	\centering
	\begin{tabular}{|p{6cm}|c|c|c|c|c|c|}
		\hline
		& \multicolumn{3}{c|}{\textbf{Wikidata Test (WD)}} & \multicolumn{3}{c|}{\textbf{TAC}} \\
		\hline
		& \multicolumn{1}{c|}{\textbf{precision}} & \multicolumn{1}{c|}{\textbf{recall}} & \multicolumn{1}{c|}{\textbf{f1}} & \multicolumn{1}{c|}{\textbf{precision}} & \multicolumn{1}{c|}{\textbf{recall}} & \multicolumn{1}{c|}{\textbf{f1}} \\
		\hline
		LR + Count Vector & 0.501 & 0.536 & 0.518 & 0.312 & 0.478 & 0.378 \\
		LR + Binary Vector & 0.502 & 0.628 & 0.558 & 0.294 & 0.590 & 0.392 \\
		LR + Sum word embedding & 0.500 & 0.516 & 0.508 & 0.290 & 0.452 & 0.353 \\
		LR + Average word embedding & 0.502 & 0.506 & 0.504 & 0.286 & 0.526 & 0.371 \\
		LR + TFIDF & 0.501 & 0.536 & 0.518 & 0.312 & 0.480 & 0.378 \\
		\hline\hline
		\SYSNAME{} (Basic+GC) &\textbf{0.826}&	\textbf{0.920}&	\textbf{0.870}&	\textbf{0.579}&	\textbf{0.812}	&\textbf{0.676}  \\
		
		%KG Cleaner with 3 layers & \textbf{0.987} & 0.813 & \textbf{0.891} & 0.289 & 0.461 & 0.355 \\
		%KG Cleaner with 4 layers & 0.982 & 0.816 & 0.891 & 0.289 & 0.461 & 0.355 \\
		\hline
	\end{tabular}%
	\caption{Credibility Performance after replacing noisy Gumbel-based models with LR ones}
	\label{tab:credibilityperformanceLR}%
\end{table*}	%


==> table/credibility_performance_naive_bayes.tex <==
% Naive Bayes included
% Table generated by Excel2LaTeX from sheet 'Credibility'
\begin{table*}[h!] \small
	\centering
	\begin{tabular}{|l|l|l|l|l|l|l|l|}
		\hline
		& \multicolumn{3}{c|}{\textbf{Wikidata Test (WD)}} & \multicolumn{3}{c|}{\textbf{TAC}} \\
		\hline
		& \multicolumn{1}{c|}{\textbf{precision}} & \multicolumn{1}{c|}{\textbf{recall}} & \multicolumn{1}{c|}{\textbf{f1}} & \multicolumn{1}{c|}{\textbf{precision}} & \multicolumn{1}{c|}{\textbf{recall}} & \multicolumn{1}{c|}{\textbf{f1}} \\
		\hline
		Naive Bayes + Count Vector & 50.08 & 58.11 & 53.80 & 28.78 & 55.65 & 37.64 \\
		Naive Bayes + Binary Vector & 50.08 & 58.11 & 53.80 & 28.78 & 55.65 & 37.64 \\
		Naive Bayes + Sum word embedding & 50 & 100 & 66.6 & 30.47 & 100.0 & 46.71 \\
		Naive Bayes + Average word embedding & 50 & 35.98 & 47.84 & 29.43 & 84.64 & 43.67 \\
		Naive Bayes + TFIDF & 50.18 & 56.37 & 53.09 & 28.92 & 56.69 & 38.30 \\
		\hline\hline
		\SYSNAME{} (Basic+GC) &\textbf{82.6}&	\textbf{92.0}&	\textbf{87.0}&	\textbf{57.9}&	\textbf{81.2}	&\textbf{67.6}  \\
		
		%KG Cleaner with 3 layers & \textbf{0.987} & 0.813 & \textbf{0.891} & 0.289 & 0.461 & 0.355 \\
		%KG Cleaner with 4 layers & 0.982 & 0.816 & 0.891 & 0.289 & 0.461 & 0.355 \\
		\hline
	\end{tabular}%
	\caption{Credibility Performance after replacing \SYSNAME{} + Gumbel + Residual Connection with Naive Bayes classifier.}
	\label{tab:credibilityperformanceNaiveBayes}%

\end{table*}	%


==> table/credibility_performance_short.tex <==
% all models included
% Table generated by Excel2LaTeX from sheet 'Credibility'
\begin{table*}[t] %\small
  \centering
  %\setlength\tabcolsep{1.7pt} % default value: 6pt
    %\resizebox{\textwidth}{!}{
    %\begin{tabular}{|p{3cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
    \begin{tabular}{|l|l|l|l|l|l|l|}
    \hline
          & \multicolumn{3}{c|}{\textbf{WD Test}} & \multicolumn{3}{c|}{\textbf{TAC}} \\
    \hline
          & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{F1}} \\
    \hline
    %LR + count vector & 0.501 & 0.536 & 0.518 & 0.312 & 0.478 & 0.378 \\
    %LR + sum word embedding & 0.500 & 0.516 & 0.508 & 0.290 & 0.452 & 0.353 \\
    %LR + TFIDF & 0.501 & 0.536 & 0.518 & 0.312 & 0.480 & 0.378 \\
    LR+Avg. Emb.           & 0.50 & 0.51 & 0.50 & 0.29 & 0.53 & 0.37 \\
    LR+Bin.                & 0.50 & 0.63 & 0.56 & 0.29 & 0.59 & 0.39 \\
    \hline\hline
    Naive Bayes + Sum Emb. & 0.50 & 1.00 & 0.66 & 0.30 & 1.0 & 0.46 \\
    Naive Bayes + Bin.     & 0.50 & 0.58 & 0.54 & 0.29 & 0.56 & 0.38 \\
    
    \hline\hline
    DistMult               & 0.58 & 0.54 & 0.56 & NA &NA &NA \\
    ComplEx                & 0.58 & 0.62 & 0.58	& NA &NA &NA\\
    \hline\hline
    MLP-1 & 0.49 & 0.99 & 0.67 &  & & \\
    MLP-2 & 0.49 & 1.00 & 0.67 & & & \\
    CNN-text & & & & &  & \\
    LSTM-text & 0.50& 0.96& 0.66& 0.30&0.99 &0.47 \\
    LSTM-text & 0.50& 0.99& 0.66& 0.30&0.99 &0.47 \\
    Declare(2018)   & 0.80& 0.99& 0.89& 0.31&0.33 &0.32 \\
    Declare(2018)   &     &     &     &     &     & \\
    \hline\hline
    %\SYSNAME{}, independent training & \textbf{0.995} & 0.820 & \textbf{0.891} & 0.299 & 0.461 & 0.355 \\
    \SYSNAME{}(Basic) & \textbf{0.98} & 0.82 & \textbf{0.89} & 0.29 & 0.46 & 0.36 \\
    %\hline\hline
    \SYSNAME{}(Basic+G)  &0.81 &	\textbf{0.94}	&0.87	&\textbf{0.59}	&\textbf{0.88}	&\textbf{0.70} \\
    %\SYSNAME{} (Shared Gumbel Noise) + outer product &0.814 &	\textbf{0.935}& 	0.870 &	\textbf{0.587} &	\textbf{0.876} &	\textbf{0.703}  \\
    \SYSNAME{}(Basic+GC) &0.83&	0.92&	0.87&	0.58&	0.81	&0.68  \\

    %KG Cleaner with 3 layers & \textbf{0.987} & 0.813 & \textbf{0.891} & 0.289 & 0.461 & 0.355 \\
    %KG Cleaner with 4 layers & 0.982 & 0.816 & 0.891 & 0.289 & 0.461 & 0.355 \\
    \hline
    \end{tabular}%
    %}
    \caption{Credibility Performance. NA (\textit{Not
        Applicable}) for DistMult and ComplEx as they train on
      fixed set of entities to generate embedding and are trained on WikiData-train, which does not overlap with TAC entities; no embeddings for TAC entities exist. }
  \label{tab:credibilityperformance}%
\end{table*}%





==> table/multi_task_vs_single_task.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet11'
\begin{table}%[htbp]
  \centering
    \begin{tabular}{|l|c|c|}
    \hline
          & \multicolumn{1}{c|}{\textbf{Wiki F1}} & \multicolumn{1}{c|}{\textbf{TAC F1}} \\
    \hline
    \textbf{cred} & \textbf{0.891} & 0.355 \\
    \textbf{multi-task cred} & 0.890 & \textbf{0.355} \\
    \hline
    \textbf{rel (micro)} & 0.771 & 0.357 \\
    \textbf{mult-task rel (micro)} & \textbf{0.791} & \textbf{0.360} \\
    \hline
    \textbf{rel (macro)} & 0.357 & 0.027 \\
    \textbf{multi-task rel (macro)} & \textbf{0.383} & \textbf{0.028} \\
    \hline
    \textbf{rel (mrr)} & 0.863 & 0.402 \\
    \textbf{multi-task rel (mrr)} & \textbf{0.871} & \textbf{0.403} \\
    \hline
    \end{tabular}%
\caption{Performance of jointly vs. individually trained models with same parameter settings.}
\label{tab:multitaskvssingaltask}%
\end{table}%



==> table/repair_performance.tex <==
% % Table generated by Excel2LaTeX from sheet 'Relation Repair'
% \begin{table*}[t]
%   \centering
%     \begin{tabular}{|c|c|c|r|r|r|r|}
%     \hline
%           & \multicolumn{3}{c|}{\textbf{Wikidata}} & \multicolumn{3}{c|}{\textbf{TAC}} \\
%     \hline
%           & \textbf{macro} & \textbf{micro} & \multicolumn{1}{l|}{\textbf{mrr}} & \multicolumn{1}{l|}{\textbf{macro}} & \multicolumn{1}{l|}{\textbf{micro}} & \multicolumn{1}{l|}{\textbf{mrr}} \\
%     \hline
%     LR + Count Vector & 0.101 & 0.054 & 0.544 & 0.020 & 0.013 & 0.607 \\
%     LR + Binary Vector & 0.163 & 0.117 & 0.555 & 0.020 & 0.035 & \textbf{0.706} \\
%     LR + Sum Word2Vec & 0.061 & 0.032 & 0.537 & 0.010 & 0.070 & 0.400 \\
%     LR + Average Word2Vec & 0.125 & 0.036 & 0.541 & 0.022 & 0.070 & 0.522 \\
%     LR + TFIDF & 0.085 & 0.279 & 0.556 & 0.004 & 0.047 & 0.493 \\
%     \hline\hline
%     KG Cleaner with 2 layers & \textbf{0.383} & \textbf{0.791} & \textbf{0.875} & \textbf{0.028} & \textbf{0.360} & 0.403 \\
%     %KG Cleaner with 3 layers & 0.364 & 0.787 & 0.872 & 0.024 & 0.359 & 0.403 \\
%     %KG Cleaner with 4 layers & \textbf{0.397} & 0.782 & \textbf{0.877} & 0.022 & 0.356 & 0.400 \\
%     \hline
%     \end{tabular}%
%   \caption{\colorbox{red}{Repair Performance when \textit{predict i.e using only class label} function of sklearn is used}}    
%   \label{tab:repairperformance}%
% \end{table*}%
% ~
\begin{table*}[t] \small
  \centering
    \begin{tabular}{|p{6.5cm}|c|c|r|r|r|r|}
    \hline
          & \multicolumn{3}{c|}{\textbf{Wikidata Test (WD) }} & \multicolumn{3}{c|}{\textbf{TAC}} \\
    \hline
          & \textbf{macro} & \textbf{micro} & \multicolumn{1}{l|}{\textbf{mrr}} & \multicolumn{1}{l|}{\textbf{macro}} & \multicolumn{1}{l|}{\textbf{micro}} & \multicolumn{1}{l|}{\textbf{mrr}} \\
    \hline
    %LR + Count Vector & 0.197 & 0.477 & 0.678 & 0.027 & 0.341 & 0.464 \\
    LR + Binary Vector & 0.194 & 0.454 & 0.678 & 0.042 & 0.648 & 0.706 \\
    %LR + Sum word embedding & 0.089 & 0.465 & 0.657 & 0.022 & 0.261 & 0.381 \\
    LR + Average word embedding & 0.124 & 0.483 & 0.687 & 0.035 & 0.607 & 0.676 \\
    %LR + TFIDF & 0.209 & 0.409 & 0.642 & 0.033 & 0.426 & 0.561 \\
    \hline\hline
    old \SYSNAME{}, independent training & 0.357 & 0.771 & 0.863 & 0.027 & 0.046 & 0.402 \\
    old \SYSNAME{} Basic & 0.383 & 0.791 & 0.875 & 0.028 & 0.360 & 0.403 \\
    \hline\hline
    %\SYSNAME{} (Shared Gumbel Noise)     &0.032	&0.500	&0.581	&0.020	&0.695	&0.712 \\
    old \SYSNAME{} (Basic+G)     &0.032	&0.500	&0.580	&0.020	&0.695	&0.712 \\
    old \SYSNAME{} (Basic+GC)    &\textbf{0.607}	&\textbf{0.889}	&\textbf{0.942}	&\textbf{0.383}	&\textbf{0.819}	&\textbf{0.866}  \\
    \hline
    new \SYSNAME{} (pytorch Basic+GC avg)     &0.6499	&0.9664	&	&0.1331	&0.3741	& \\
    \end{tabular}%
  \caption{Repair Performance. Macro and Micro are F1 scores.  }%when \textit{predict\_proba i.e using probability} function of sklearn is used}    
  \label{tab:repairperformance}%
\end{table*}%
    %KG Cleaner with 3 layers & 0.364 & 0.787 & 0.872 & 0.024 & 0.359 & 0.403 \\
%KG Cleaner with 4 layers & \textbf{0.397} & 0.782 & \textbf{0.877} & 0.022 & 0.356 & 0.400 \\


==> table/repair_performanceLR.tex <==
\begin{table*}[t] \small
  \centering
    \begin{tabular}{|p{6.5cm}|c|c|r|r|r|r|}
    \hline
          & \multicolumn{3}{c|}{\textbf{Wikidata Test (WD) }} & \multicolumn{3}{c|}{\textbf{TAC}} \\
    \hline
          & \textbf{macro} & \textbf{micro} & \multicolumn{1}{l|}{\textbf{mrr}} & \multicolumn{1}{l|}{\textbf{macro}} & \multicolumn{1}{l|}{\textbf{micro}} & \multicolumn{1}{l|}{\textbf{mrr}} \\
    \hline
    MaxEnt + Count Vector & 0.197 & 0.477 & 0.678 & 0.027 & 0.341 & 0.464 \\
    MaxEnt + Binary Vector & 0.194 & 0.454 & 0.678 & 0.042 & 0.648 & 0.706 \\
    MaxEnt + Sum word embedding & 0.089 & 0.465 & 0.657 & 0.022 & 0.261 & 0.381 \\
    MaxEnt + Average word embedding & 0.124 & 0.483 & 0.687 & 0.035 & 0.607 & 0.676 \\
    MaxEnt + TFIDF & 0.209 & 0.409 & 0.642 & 0.033 & 0.426 & 0.561 \\
    \hline\hline
    %MLP, independent training & 0.357 & 0.771 & 0.863 & 0.027 & 0.046 & 0.402 \\
    %\SYSNAME{} with 2 layers & 0.383 & 0.791 & 0.875 & 0.028 & 0.360 & 0.403 \\
    %\hline\hline
    %\SYSNAME{} (Shared Gumbel Noise)     &0.032	&0.500	&0.581	&0.020	&0.695	&0.712 \\
    %\SYSNAME{} (Shared Gumbel Noise) + outer product     &0.032	&0.500	&0.580	&0.020	&0.695	&0.712 \\
    \SYSNAME{} (Basic+GC)    &\textbf{0.607}	&\textbf{0.889}	&\textbf{0.942}	&\textbf{0.383}	&\textbf{0.819}	&\textbf{0.866}  \\
    \hline
    \end{tabular}%
  \caption{Repair Performance after replacing noisy Gumbel-based
    models with Maximum Entropy model (MaxEnt) ones. Macro and Micro are F1 scores.  }%when \textit{predict\_proba i.e using probability} function of sklearn is used}    
  \label{tab:repairperformanceLR}%
\end{table*}%


==> table/repair_performance_naive_bayes.tex <==
\begin{table*}[h!] \small
  \centering
    \begin{tabular}{|p{6.5cm}|c|c|r|r|r|r|}
    \hline
          & \multicolumn{3}{c|}{\textbf{Wikidata Test (WD) }} & \multicolumn{3}{c|}{\textbf{TAC}} \\
    \hline
          & \textbf{macro} & \textbf{micro} & \multicolumn{1}{l|}{\textbf{mrr}} & \multicolumn{1}{l|}{\textbf{macro}} & \multicolumn{1}{l|}{\textbf{micro}} & \multicolumn{1}{l|}{\textbf{mrr}} \\
    \hline
    Naive Bayes + Count Vector & 12.67 & 36.58 & 57.39 & 4.16 & 12.7 & 38.36 \\
    Naive Bayes + Binary Vector & 12.67 & 36.58 & 57.39 & 4.16 & 12.7 & 38.36 \\
    Naive Bayes + Sum word embedding & 3.14 & 5.2 & 16.55 & 10.80 & 21.58 & 6.06 \\
    Naive Bayes + Average word embedding & 9.23 & 30.18 & 46.05 & 11.07 & 11.06 & 24.93 \\
    Naive Bayes + TFIDF & 1.413 & 30.96 & 68.66 & 1.313 & 9.26 & 71.02 \\
    \hline\hline
    %MLP, independent training & 0.357 & 0.771 & 0.863 & 0.027 & 0.046 & 0.402 \\
    %\SYSNAME{} with 2 layers & 0.383 & 0.791 & 0.875 & 0.028 & 0.360 & 0.403 \\
    %\hline\hline
    %\SYSNAME{} (Shared Gumbel Noise)     &0.032	&0.500	&0.581	&0.020	&0.695	&0.712 \\
    %\SYSNAME{} (Shared Gumbel Noise) + outer product     &0.032	&0.500	&0.580	&0.020	&0.695	&0.712 \\
    \SYSNAME{} (Basic+GC) &\textbf{60.7}	&\textbf{88.9}	&\textbf{94.2}	&\textbf{38.3}	&\textbf{81.9}	&\textbf{86.6}  \\
    \hline
    \end{tabular}%
  \caption{Repair Performance after replacing \SYSNAME{} + Gumbel + Residual Connection models with Naive Bayes ones. Macro and Micro are F1 scores.  }%when \textit{predict\_proba i.e using probability} function of sklearn is used}    
  \label{tab:repairperformanceNaiveBayes}%
\end{table*}%


==> table/repair_performance_new.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
	\centering
	\resizebox{0.99\textwidth}{!}{
	\begin{tabular}{|c|c|c|c||c|c|c||c|c|c||c|c|c|}
		\hline
			\textbf{Rep.} & \textbf{Comb.} & \textbf{Clf.} & \textbf{Skip} & \multicolumn{3}{c||}{\textbf{TACRED}} & \multicolumn{3}{c||}{\textbf{TAC-2017}} & \multicolumn{3}{c|}{\textbf{TAC-2015}} \\
		\hline
			& & &  & \textbf{Macro} & \textbf{Micro} & \textbf{MRR} & \textbf{Macro} & \textbf{Micro} & \textbf{MRR} & \textbf{Macro} & \textbf{Micro} & \textbf{MRR} \\
		\hline		\hline
		%\textbf{Model} & \multicolumn{1}{p{4.055em}|}{\textbf{macro }} & \multicolumn{1}{p{4.055em}|}{\textbf{micro }} & \multicolumn{1}{p{4.055em}|}{\textbf{mrr }} & \multicolumn{1}{p{4.055em}|}{\textbf{macro }} & \multicolumn{1}{p{4.055em}|}{\textbf{micro }} & \multicolumn{1}{p{4.055em}|}{\textbf{mrr }} & \multicolumn{1}{p{4.055em}|}{\textbf{macro }} & \multicolumn{1}{p{4.055em}|}{\textbf{micro }} & \multicolumn{1}{p{4.055em}|}{\textbf{mrr }} \\
		%\textbf{LR+Count} & 15.60 & 42.16 & 0.82  & 43.06 & 48.29 & 0.73  & 42.10 & 47.51 & 0.73 \\
		%\hline
		%\textbf{LR+Binary} & 15.61 & 42.20 & 0.82  & 43.11 & 48.33 & 0.73  & 42.11 & 47.51 & 0.73 \\
		%\hline
		\textbf{TF-IDF} & No & LR & No & \textbf{14.50} & 43.48 & 0.83  & 75.49 & 76.80 & 0.76  & \textbf{76.35} & \textbf{77.57} & 0.76 \\
		%\hline
		%\textbf{LR+Emb.+SUM} & 4.06  & 41.79 & 0.83  & 2.67  & 16.51 & 0.69  & 7.55  & 20.11 & 0.70 \\
		%\hline
		%\textbf{LR+Emb.+AVG} & 5.01  & 42.21 & \textbf{0.84}  & 7.38  & 20.14 & 0.71  & 2.79  & 16.74 & 0.69 \\
		%\hline		\hline
		%\textbf{NB+Count} & 11.15 & 37.89 & 0.82  & 66.85 & 68.52 & 0.83  & 12.82 & 24.48 & 0.72 \\
		%\hline
		%\textbf{NB+Binary} & 11.15 & 37.89 & 0.82  & 66.85 & 68.52 & 0.83  & 12.82 & 24.48 & 0.72 \\
		%\hline
		\textbf{Binary} & No & NB & No  & 2.17  & 41.66 & 0.83  & 67.72 & 70.37 & 0.85  & 2.14  & 16.26 & 0.71 \\
		%\hline
		%\textbf{NB+Emb.+SUM} & 12.42 & 13.15 & 0.34  & 35.04 & 36.88 & 0.53  & 32.54 & 33.78 & 0.63 \\
		%\hline
		%\textbf{NB+Emb.+AVG} & \textbf{18.84} & 22.84 & 0.59  & 35.84 & 37.57 & 0.64  & 35.51 & 36.23 & 0.43 \\
		\hline
		\hline
		$\spadesuit$ \textbf{LSTM} & No & MLP & No & 1.87  & 78.56 & 0.82  & 3.05  & 33.04 & 0.53  & 1.46  & 61.30 & 0.68 \\
		\hline
		$\spadesuit$ \textbf{Bi-LSTM} & Yes (W) & MLP & No & 1.87  & 78.56 & 0.81  & 0.20  & 7.38  & 0.27  & 1.46  & 61.30 & 0.66 \\
		\hline		\hline
		\textbf{BERT} & Yes (S) & MLP & Yes & 6.17  & 16.43  & 0.29    & 70.95  & 80.43 & 0.89  &   56.74  & 62.36  & 0.73 \\
		\hline
		\textbf{BoW embedding} & Yes (S) & MLP & Yes & 2.10  & \textbf{78.56} & 0.81  & \textbf{79.13} & \textbf{84.15} & \textbf{0.91} & 64.90 & 75.90 & \textbf{0.85} \\
		%\textbf{\SYSNAME}(LSTM) & 1.38& 21.33& 0.37 & & &  & 0.71 & 3.22 & 0.14 \\
%\hline\hline
%\textbf{\SYSNAME}+nothing & 0.02 & 0.52 & 0.05 &0.02 &0.16 & 0.06 & 0.03 & 0.52 & 0.05 \\
%\textbf{\SYSNAME}+C & 0.01 & 0.24 & 0.05 & 0.01 & 0.17 & 0.06  & 0.07 & 0.45 & 0.11\\
%\textbf{\SYSNAME}+A & 0.55 & 0.81 & 0.06 & 1.41 & 6.26 & 0.20 &0.28 & 0.48 & 0.06 \\
%\textbf{\SYSNAME}+T & 0.37 & 0.78  & 0.08  & 1.10  & 3.65  & 0.10 & 0.9 & 6.05 & 0.19  \\
%\textbf{\SYSNAME}+A+T & 2.10  & \textbf{78.56} & 0.81  & \textbf{79.13} & \textbf{84.15} & \textbf{0.91} & 64.90 & 75.90 & \textbf{0.85} \\
		\hline
	\end{tabular}%
}
	\caption{Repair Performance of models with abbreviations as in Table \ref{tab:consistencyPerformance}.}

	\label{tab:repairPerformance}%
\end{table*}%


==> table/repair_performance_short.tex <==
% % Table generated by Excel2LaTeX from sheet 'Relation Repair'
% \begin{table*}[t]
%   \centering
%     \begin{tabular}{|c|c|c|r|r|r|r|}
%     \hline
%           & \multicolumn{3}{c|}{\textbf{Wikidata}} & \multicolumn{3}{c|}{\textbf{TAC}} \\
%     \hline
%           & \textbf{macro} & \textbf{micro} & \multicolumn{1}{l|}{\textbf{mrr}} & \multicolumn{1}{l|}{\textbf{macro}} & \multicolumn{1}{l|}{\textbf{micro}} & \multicolumn{1}{l|}{\textbf{mrr}} \\
%     \hline
%     LR + Count Vector & 0.101 & 0.054 & 0.544 & 0.020 & 0.013 & 0.607 \\
%     LR + Binary Vector & 0.163 & 0.117 & 0.555 & 0.020 & 0.035 & \textbf{0.706} \\
%     LR + Sum Word2Vec & 0.061 & 0.032 & 0.537 & 0.010 & 0.070 & 0.400 \\
%     LR + Average Word2Vec & 0.125 & 0.036 & 0.541 & 0.022 & 0.070 & 0.522 \\
%     LR + TFIDF & 0.085 & 0.279 & 0.556 & 0.004 & 0.047 & 0.493 \\
%     \hline\hline
%     KG Cleaner with 2 layers & \textbf{0.383} & \textbf{0.791} & \textbf{0.875} & \textbf{0.028} & \textbf{0.360} & 0.403 \\
%     %KG Cleaner with 3 layers & 0.364 & 0.787 & 0.872 & 0.024 & 0.359 & 0.403 \\
%     %KG Cleaner with 4 layers & \textbf{0.397} & 0.782 & \textbf{0.877} & 0.022 & 0.356 & 0.400 \\
%     \hline
%     \end{tabular}%
%   \caption{\colorbox{red}{Repair Performance when \textit{predict i.e using only class label} function of sklearn is used}}    
%   \label{tab:repairperformance}%
% \end{table*}%
% ~
\begin{table*}[t] \small
  \centering
  \setlength\tabcolsep{1.7pt} % default value: 6pt


    \begin{tabular}{|p{3.1cm}|p{0.83cm}|p{0.8cm}|p{0.6cm}|p{0.83cm}|p{0.8cm}|p{0.6cm}|}
    \hline
          & \multicolumn{3}{c|}{\textbf{WD Test}} & \multicolumn{3}{c|}{\textbf{TAC}} \\
    \hline
          & \textbf{macro} & \textbf{micro} & \textbf{mrr} & \textbf{macro} & \textbf{micro} & \textbf{mrr}\\
    \hline
    %LR + Count Vector & 0.197 & 0.477 & 0.678 & 0.027 & 0.341 & 0.464 \\
    LR + Bin. & 0.19 & 0.45 & 0.68 & 0.04 & 0.65 & 0.71 \\
    %LR + Sum word embedding & 0.089 & 0.465 & 0.657 & 0.022 & 0.261 & 0.381 \\
    LR + Ag. Emb.& 0.12 & 0.48 & 0.69 & 0.04 & 0.61 & 0.68 \\
    %LR + TFIDF & 0.209 & 0.409 & 0.642 & 0.033 & 0.426 & 0.561 \\
    \hline\hline
    %\SYSNAME{}, independent training & 0.357 & 0.771 & 0.863 & 0.027 & 0.046 & 0.402 \\
    \SYSNAME{}(Basic) & 0.38 & 0.79 & 0.88 & 0.03 & 0.36 & 0.40 \\
%    \hline\hline
    \SYSNAME{}(Basic+G)  &0.03	&0.50	&0.58	&0.02	&0.70	&0.71 \\
    %\SYSNAME{} (Shared Gumbel Noise) + outer product     &0.032	&0.500	&0.580	&0.020	&0.695	&0.712 \\
    \SYSNAME{}(Basic+GC) &\textbf{0.61}	&\textbf{0.89}	&\textbf{0.94}	&\textbf{0.38}	&\textbf{0.82}	&\textbf{0.87}  \\
    \hline
    \end{tabular}%
  \caption{Repair Performance. Macro and Micro are F1 scores.  }%when \textit{predict\_proba i.e using probability} function of sklearn is used}    
  \label{tab:repairperformance}%
\end{table*}%
    %KG Cleaner with 3 layers & 0.364 & 0.787 & 0.872 & 0.024 & 0.359 & 0.403 \\
%KG Cleaner with 4 layers & \textbf{0.397} & 0.782 & \textbf{0.877} & 0.022 & 0.356 & 0.400 \\


==> table/wikidata_relation.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
  \centering
  \begin{scriptsize}
    %\begin{tabular}{ccccc}
    \begin{tabular}{|lllll|}
      \hline
    affiliation & child & educated at & member of political party & parent club \\
    
    alternate names & convicted of & end time & mother & parent organization \\
    
    birthday & country of origin & ethnic group & noble title & place of birth \\
    
    birth name & crew member & father & number of seats & place of death \\
    
    board member & date of birth & founded by & occupant & political alignment \\
    
    business division & date of burial orcremation & inception & official name & posthumous name \\
    
    capital & date of death & manner of death & official residence & reference URL \\
    
    cause of death & discontinued date & member count & official website & religion \\
    
    charge & dissolved, abolished or demolished & member of & owned by & residence \\
    
    sibling & spouse & subsidiary &       &  \\
    \hline
    \end{tabular}%
    \end{scriptsize}
    \caption{Wikidata relationships considered for credibility and repair.}
  \label{tab:wikidata_relations}%
 
\end{table*}%

